Top Ten Challenges Towards Agentic Neural Graph Databases

Graph databases (GDBs) like Neo4j and TigerGraph excel at handling interconnected data but lack advanced inference capabilities. Neural Graph Databases (NGDBs) address this by integrating Graph Neural Networks (GNNs) for predictive analysis and reasoning over incomplete or noisy data. However, NGDBs rely on predefined queries and lack autonomy and adaptability. This paper introduces Agentic Neural Graph Databases (Agentic NGDBs), which extend NGDBs with three core functionalities: autonomous query construction, neural query execution, and continuous learning. We identify ten key challenges in realizing Agentic NGDBs: semantic unit representation, abductive reasoning, scalable query execution, and integration with foundation models like large language models (LLMs). By addressing these challenges, Agentic NGDBs can enable intelligent, self-improving systems for modern data-driven applications, paving the way for adaptable and autonomous data management solutions.

==> sec_query_language.tex <==
% \section{What queries can we support?}

% There are no assumptions about the constant and under them.

% \begin{itemize}
%     \item current stage: tree-formed/efo1/efok
%     \item more advanced ones: SQL, SPARQL, OWL, N-arity=2 of predicate / K-arity of answers
% \end{itemize}

\vspace{-.5em}
\section{Challenge 2: Query Expressiveness}
\vspace{-.5em}

% In this section, we explore the extent to which complex queries have been investigated in the graph databases and how the query family has evolved over the years. To this end, we discuss the query expressiveness by several progressively larger query families, specifically, we introduce three query families that have already been put forward in the current research stage:

% %\subsection{Investigated query family}


% \textbf{(1) Tree-formed query:}
% The tree-formed query is a collective term that describes the whole query family that can be recursively defined in a tree structure. The definition of tree-formed query is entangled with the development of query embedding methods, as will be detailed later. % The development of such methodology helps to support more and more set operations, from set projection~\cite{NGDB:hamilton_embedding_2018}, intersection, union~\cite{NGDB:ren_query2box_2020}, complement\cite{NGDB:ren_query2box_2020} and set difference~\cite{NGDB:liu_neural-answering_2021}.
% \textbf{(2) EFO-1 query:}
% It is shown that tree-formed query family is constrained by certain assumptions and fails to represent Existential First Order queries with one free variable (EFO-1 query) such as cyclic query~\cite{NGDB:yin_rethinking_2023}. It is also shown that the whole query family of EFO-1 is fundamentally more complex than the tree-formed query: regarding the query complexity, EFO-1 is NP-complete while the tree-formed query is polynomial. 
% \textbf{(3) EFO-$k$ query:}
% Researchers further extended to answer queries from one single free variable with $k$ free variables~\cite{NGDB:yin_textefo_k-cqa_2023}, and each answer of such query should be a $k$-ary tuple. This put forward great challenges to existing methods as the search space for answers grows exponentially, and the current model fails to explore the combinatorial hardness. 



Previous research only studies NGDB queries from a small fragment of the logical query family supported by traditional database query languages such as SQL or SPARQL. For example, the tree-formed query family that includes set operations~\cite{NGDB:wang_benchmarking_2021} and the EFO-1~\cite{NGDB:yin_rethinking_2023} and EFO-$k$~\cite{NGDB:yin_textefo_k-cqa_2023} query families that target general existential first-order formulas. This is because the progress in NGDB is largely biased by the inductive biases of neural networks, which will be detailed in Challenge 4.


% \textbf{More advanced query types.}
More advanced query families still exist, though research on these topics is insufficient at the current stage. Thus, we discuss some of the challenges we might face in pursuit of more advanced queries in NGDB from the following aspects
\textbf{(i) Multi-arity predicates:}
The first challenge we may encounter is when the knowledge databases are constructed by $(n+1)$-ary tuples, the relation corresponds to $n$-ary predicate and a graph becomes a hypergraph~\cite{NGDB:luo_nqe_2022}.
% Another challenge is the attributes of entities and relations which are largely undiscussed, the attributes can be categorical~\citep{hu_type-aware_2022} or numerical~\citep{DBLP:conf/kdd/BaiLLYYS23}.
% These features are largely unexplored, leading to the consequence that current query expressiveness is strictly limited compared to database-level query languages . 
\textbf{(ii) Support of functions}
The corresponding research gap is the support for functions in the query -- a function can output nodes, numbers, semantic units, or data of more advanced modality -- for example, the ``AVG'' and ``COUNT'' functions in SQL but not in current CQA models. We have noted one preliminary research trying to fill this gap~\cite{NGDB:DBLP:conf/pkdd/DemirWLNH23}.
% Another drawback is that the current model only returns a ranking for all entities in the graph rather than a classification result telling whether an answer is true or false. This leads to the issue of counting the size of answers when we are more interested in the number of answers rather than listing some favorable answers.

